Phase-Mapper: An AI Platform to Accelerate High Throughput Materials Discovery

High-Throughput materials discovery involves the rapid synthesis, measurement, and characterization of many different but structurally-related materials. A key problem in materials discovery, the phase map identification problem, involves the determination of the crystal phase diagram from the materials' composition and structural characterization data. We present Phase-Mapper, a novel AI platform to solve the phase map identification problem that allows humans to interact with both the data and products of AI algorithms, including the incorporation of human feedback to constrain or initialize solutions. Phase-Mapper affords incorporation of any spectral demixing algorithm, including our novel solver, AgileFD, which is based on a convolutive non-negative matrix factorization algorithm. AgileFD can incorporate constraints to capture the physics of the materials as well as human feedback. We compare three solver variants with previously proposed methods in a large-scale experiment involving 20 synthetic systems, demonstrating the efficacy of imposing physical constrains using AgileFD. Phase-Mapper has also been used by materials scientists to solve a wide variety of phase diagrams, including the previously unsolved Nb-Mn-V oxide system, which is provided here as an illustrative example.

==> Makefile <==
.PHONY: main fromscratch dvi ps pdf bibs xfigs compact clean tar tgz

TEXFILE    = Agile_Materials_Platform

LATEX      = latex
BIBTEX     = bibtex
MAKEINDEX  = makeindex
DVIPS      = dvips -t letter
PDFLATEX   = pdflatex
PS2PDF     = ps2pdf
XFIGDIR     = xfigs
CURRENTDIR = `basename "\`pwd\`"`

default: pdf

#fromscratch: xfigs
fromscratch:
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(LATEX) $(TEXFILE)
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

dvi:
	$(LATEX) $(TEXFILE)

ps: dvi
	$(DVIPS) $(TEXFILE).dvi -o $(TEXFILE).ps

pdf:
	$(PDFLATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
	$(PDFLATEX) $(TEXFILE)
#pdf: ps
#$(PS2PDF) $(TEXFILE)

bibs:
	$(BIBTEX) $(TEXFILE)

xfigs:
	(cd $(FIGDIR); bash ./makefigs ../*.tex )

compact:
#	(rm -f *.aux *.log *.blg *.out *.toc $(TEXFILE).bbl)
	(rm -f *.aux *.log *.blg *.out *.toc)

clean: compact
#	(rm -f *.dvi *.ps *.pdf $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )
	(rm -f *.dvi *.ps *.pdf $(TEXFILE).bbl $(FIGDIR)/*.{eps,pdf,pstex,pstex_t,fig.bak} )

tar:
	rm -f ../$(CURRENTDIR).tar.gz
	tar cvf ../$(CURRENTDIR).tar ../$(CURRENTDIR)
	gzip ../$(CURRENTDIR).tar
	echo "Created ../$(CURRENTDIR).tar.gz"

tgz:
	rm -f ../$(CURRENTDIR).tgz
	tar cvfz ../$(CURRENTDIR).tgz ../$(CURRENTDIR)
	echo "Created ../$(CURRENTDIR).tgz"



==> NbVMnsuppinfo.tex <==
\subsubsection{Case Study: Solution comparison for Nb-V-Mn oxide system}
To further compare the impact of imposing \textit{a priori} constraints in AgileFD, we compare the phase concentration-shifting maps in Figure \ref{fig:compareshifts} and the basis patterns in Figure \ref{fig:comparebasis}. The number of similarities between the solutions in Figure \ref{fig:compareshifts} indicate that convolutional NMF is able to capture several important aspects of the phase map. However,, important differences between the concentration maps of each of the first 2 phases highlights that imposing Gibbs phase rule in AgileFD fundamentally changes the solution in ways that cannot be mimicked by post-modification of the convolutional NMF solution. That is, the map of the number of phases in Figure \ref{fig:numphases} is obtained by counting, for each sample, the number of phases with finite concentration in Figure \ref{fig:compareshifts}. Gibbs phase rule could be applied to the convolutional NMF solution by only utilizing the 3 most prominent phases at each sample point, but inspection of Figure \ref{fig:compareshifts} reveals that this yields a much different phase map than that provided by AgileFD.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.95\linewidth]{figs/compareshifts_v1}
  \caption{Phase map representation of $H$ for the convolutional NMF solution (top) and the AgileFD solution (bottom). For each basis phase, the composition plot shows the composition samples containing the phase with point size indicating the concentration of the phase and the point color indicating the fractional shift with respect to the plotted basis patterns. The elemental labels for the composition diagrams are shown in Figure \ref{fig:numphases}.}  \label{fig:compareshifts}
\end{figure}

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.95\linewidth]{figs/comparebasis_v1}
  \caption{ The $K$=6 basis patterns from $W$ for the AgileFD solution (left) and convolutional NMF solution (right) to the Nb-V-Mn system are shown along with the stick patterns (translucent red) of the phases that were identified using the AgileFD solution. The primary discrepancy between a basis pattern and that of the identified phase is highlighted.}
  \label{fig:comparebasis}
\end{figure}


The important differences between the convolutional NMF and AgileFD solutions is also apparent in the basis patterns. While several notable differences are found, the most prominent difference is in the second basis pattern where the convolutional NMF basis pattern is quite different from the AgileFD solution. This convolutional NMF basis pattern contains a mixture of signals from other phases and is thus not able to be matched to a known structure. The researcher would thus be left with the impression that this may be a newly discovered phase and undergo the arduous task of hypothesizing new crystal structures that could correspond to this basis pattern. The false-positive phase discovery from convolutional NMF is circumvented in the AgileFD solution as the encoding of Gibbs phase rule in the solver results in effective de-mixing of basis patterns such that all 6 primary phases are identified.


==> freeze.tex <==
%\section{Freezing}


